Markov Abstractions for PAC Reinforcement Learning in Non-Markov Decision Processes

Our work aims at developing reinforcement learning algorithms that do not rely on the Markov assumption. We consider the class of Non-Markov Decision Processes where histories can be abstracted into a finite set of states while preserving the dynamics. We call it a Markov abstraction since it induces a Markov Decision Process over a set of states that encode the non-Markov dynamics. This phenomenon underlies the recently introduced Regular Decision Processes (as well as POMDPs where only a finite number of belief states is reachable). In all such kinds of decision process, an agent that uses a Markov abstraction can rely on the Markov property to achieve optimal behaviour. We show that Markov abstractions can be learned during reinforcement learning. Our approach combines automata learning and classic reinforcement learning. For these two tasks, standard algorithms can be employed. We show that our approach has PAC guarantees when the employed algorithms have PAC guarantees, and we also provide an experimental evaluation.

==> sections/experimental-details.tex <==

\section{Experimental evaluation details}
\label{sec:experimental-details}

We first highlight that the implementation used in the experiments is not entirely aligned 
with the descriptions given in Appendix \ref{sec:algorithm-pseudocodes}. 
The differences are not intentional and it can be easily aligned. 
There are two differences. 
First, our implementation of \texttt{StreamCPDFALearner} assumes that transitions depend 
on observations only. 
The assumption is valid in the considered domains. 
It gives some extra help because the algorithm generates fewer candidates. 
Second, our implentation of \texttt{RMax} agent assumes that the termination probability 
is constant and provided as part of the input. 
As pointed out in the preliminaries, a constant termination probability $1-\gamma$ amounts 
to a discount factor $\gamma$, which has to be taken into account during the computation of 
the value function. 
Again, the assumption is valid in the considered domains and gives some extra help. 

We now report and discuss the parameters used in the experimental evaluation in Table~\ref{tab:domain-parameters}. 
The table is segmented in three parts. 
First, \textit{Domain parameters} shows the set of parameters that configure the domain in each experiment. 
Second, \textit{RMax parameters} shows the the discount factor $\gamma$ and $V_{max}$ used by the Markov agent. 
Note that \textit{RMax parameters} reports the values used by \texttt{RMax} as a baseline and by \texttt{RMax} as 
the Markov agent interacting with the \texttt{MarkovAbstraction}.
Third, \textit{Markov Abstraction parameters} shows the values for distinguishability $\mu$, delay $d$, 
an upper bound on the number of states $n$, and the exploration policy. 
The parameters shown in this table are domain-specific, and the parameters that configure 
the domains follow the ones introduced in \cite{abadi2020learning}.


\begin{table}[h]
    \centering
    \scriptsize
    \begin{tabular}{@{}rllrrrrrrl@{}}
    \multicolumn{10}{c}{\textbf{Rotating MAB}}                                                                                                                                                                                                                                                                                                                                                            \\ \hline
    \multicolumn{4}{|c|}{\textbf{Domain parameters}}                                                                                                                & \multicolumn{2}{c|}{\textbf{RMax parameters}}                            & \multicolumn{4}{c|}{\textbf{Markov Abstraction   parameters}}                                                                                            \\ \hline
    \multicolumn{1}{|r|}{$k$} & \multicolumn{2}{l|}{\textit{Arm probabilities}}                                       & \multicolumn{1}{r|}{\textit{Reward}} & \multicolumn{1}{r|}{$\gamma$} & \multicolumn{1}{r|}{$V_{max}$} & \multicolumn{1}{r|}{$\mu$} & \multicolumn{1}{r|}{$d$} & \multicolumn{1}{r|}{$n$} & \multicolumn{1}{l|}{\textit{Sampling policy}} \\ \hline
    \multicolumn{1}{|r|}{2}          & \multicolumn{2}{l|}{{[}0.9, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.35}        & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{3}          & \multicolumn{2}{l|}{{[}0.9, 0.2, 0.2{]}}                                              & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.23}        & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{4}          & \multicolumn{2}{l|}{{[}0.9, 0.2, 0.2, 0.2{]}}                                         & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.175}       & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{5}          & \multicolumn{2}{l|}{{[}0.9, 0.2, 0.2, 0.2, 0.2{]}}                                    & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.14}        & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{6}          & \multicolumn{2}{l|}{{[}0.9, 0.2, 0.2, 0.2, 0.2, 0.2{]}}                               & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.116}       & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline \addlinespace[0.1cm]
    \multicolumn{10}{c}{\textbf{Malfunction MAB}}                                                                                                                                                                                                                                                                                                                                                         \\ \hline
    \multicolumn{4}{|c|}{\textbf{Domain parameters}}                                                                                                                & \multicolumn{2}{c|}{\textbf{RMax parameters}}                            & \multicolumn{4}{c|}{\textbf{Markov Abstraction   parameters}}                                                                                            \\ \hline
    \multicolumn{1}{|r|}{$k$} & \multicolumn{2}{l|}{\textit{Arm probabilities}}                                       & \multicolumn{1}{r|}{\textit{Reward}} & \multicolumn{1}{r|}{$\gamma$} & \multicolumn{1}{r|}{$V_{max}$} & \multicolumn{1}{r|}{$\mu$} & \multicolumn{1}{r|}{$d$} & \multicolumn{1}{r|}{$n$} & \multicolumn{1}{l|}{\textit{Sampling policy}} \\ \hline
    \multicolumn{1}{|r|}{3}          & \multicolumn{2}{l|}{{[}0.8, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.079}       & \multicolumn{1}{r|}{4}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{3}          & \multicolumn{2}{l|}{{[}0.8, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.31}        & \multicolumn{1}{r|}{4}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Single random action}     \\ \hline
    \multicolumn{1}{|r|}{5}          & \multicolumn{2}{l|}{{[}0.8, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.2047}      & \multicolumn{1}{r|}{6}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Single random action}     \\ \hline \addlinespace[0.1cm]
    \multicolumn{10}{c}{\textbf{Cheat MAB}}                                                                                                                                                                                                                                                                                                                                                               \\ \hline
    \multicolumn{4}{|c|}{\textbf{Domain parameters}}                                                                                                                & \multicolumn{2}{c|}{\textbf{RMax parameters}}                            & \multicolumn{4}{c|}{\textbf{Markov Abstraction   parameters}}                                                                                            \\ \hline
    \multicolumn{1}{|r|}{$k$} & \multicolumn{2}{l|}{\textit{Arm probabilities}}                                       & \multicolumn{1}{r|}{\textit{Reward}} & \multicolumn{1}{r|}{$\gamma$} & \multicolumn{1}{r|}{$V_{max}$} & \multicolumn{1}{r|}{$\mu$} & \multicolumn{1}{r|}{$d$} & \multicolumn{1}{r|}{$n$} & \multicolumn{1}{l|}{\textit{Sampling policy}} \\ \hline
    \multicolumn{1}{|r|}{3}          & \multicolumn{2}{l|}{{[}0.2, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.049}       & \multicolumn{1}{r|}{4}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline
    \multicolumn{1}{|r|}{4}          & \multicolumn{2}{l|}{{[}0.2, 0.2{]}}                                                   & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.909}          & \multicolumn{1}{r|}{1098.9}        & \multicolumn{1}{r|}{0.0254}      & \multicolumn{1}{r|}{5}              & \multicolumn{1}{r|}{10}         & \multicolumn{1}{l|}{Uniform random}           \\ \hline \addlinespace[0.1cm]
    \multicolumn{10}{c}{\textbf{Rotating Maze}}                                                                                                                                                                                                                                                                                                                                                           \\ \hline
    \multicolumn{4}{|c|}{\textbf{Domain parameters}}                                                                                                                & \multicolumn{2}{c|}{\textbf{RMax parameters}}                            & \multicolumn{4}{c|}{\textbf{Markov Abstraction   parameters}}                                                                                            \\ \hline
    \multicolumn{1}{|r|}{$k$} & \multicolumn{1}{l|}{\textit{Grid size}} & \multicolumn{1}{l|}{\textit{Goal position}} & \multicolumn{1}{r|}{\textit{Reward}} & \multicolumn{1}{r|}{$\gamma$} & \multicolumn{1}{r|}{$V_{max}$} & \multicolumn{1}{r|}{$\mu$} & \multicolumn{1}{r|}{$d$} & \multicolumn{1}{r|}{$n$} & \multicolumn{1}{l|}{\textit{Sampling policy}} \\ \hline
    \multicolumn{1}{|r|}{1}          & \multicolumn{1}{l|}{4x4}                & \multicolumn{1}{l|}{(2, 3)}                 & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.9375}         & \multicolumn{1}{r|}{100}           & \multicolumn{1}{r|}{0.224}       & \multicolumn{1}{r|}{1}              & \multicolumn{1}{r|}{100}        & \multicolumn{1}{l|}{Single random action}     \\ \hline
    \multicolumn{1}{|r|}{2}          & \multicolumn{1}{l|}{4x4}                & \multicolumn{1}{l|}{(2, 3)}                 & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.9375}         & \multicolumn{1}{r|}{100}           & \multicolumn{1}{r|}{0.2}         & \multicolumn{1}{r|}{2}              & \multicolumn{1}{r|}{150}        & \multicolumn{1}{l|}{Single random action}     \\ \hline
    \multicolumn{1}{|r|}{3}          & \multicolumn{1}{l|}{4x4}                & \multicolumn{1}{l|}{(2, 3)}                 & \multicolumn{1}{r|}{100}             & \multicolumn{1}{r|}{0.9375}         & \multicolumn{1}{r|}{100}           & \multicolumn{1}{r|}{0.18}        & \multicolumn{1}{r|}{3}              & \multicolumn{1}{r|}{200}        & \multicolumn{1}{l|}{Single random action}     \\ \hline \addlinespace[0.1cm]
    \end{tabular}
    \caption{Domain-specific parameters.}
    \label{tab:domain-parameters}
\end{table}


The distinguishability $\mu$ and the upper bound on the number of states $n$ are strictly domain-dependent.
On the one hand, the value for distinguishability needs to be computed taking into consideration the probabilities 
that define the domain dynamics, such that it reflects the probability of sampling distinguishing histories. 
On the other hand, the upper bound on the number of states needs to consider the actual number of safe 
states that compose the hypothesis MDP. 
It is possible to approximately compute these values when domain knowledge is available, and the values 
we show are approximated manually for each domain. 
Note that, if domain knowledge is not available, one can employ a search strategy for finding values 
for these parameters, as discussed in Appendix \ref{sec:algorithm-pseudocodes}. 

The delay $d$ and the exploration policy, i.e. the length of histories that must be considered 
in order to distinguish a states and the policy that samples histories, have direct impact on the 
required value for distinguishability. 
As the necessary length of a history increases, the probability of sampling distinguishing histories decreases. 
Under the uniform random policy, the probability of sampling a history is affected both by the required delay and 
by the number of actions in the domain. 
This is exemplified in the Cheat MAB domain, where the distinguishability value is approximately halved 
with an increase in delay of $+1$. 
In domains where the single random action policy is applicable, the probability of histories do not 
decrease as much as with the uniform policy, due to the fact that the action is fixed. 
One example is in the Rotating Maze domain experiments, where increasing the delay mildly affects the values 
used for distinguishability under the single random action policy. 
Note that the single random action policy is particularly distinguishing in the domains that we employed it, 
but not in general. 

The maximum value $V_{max}$ used in each domain needs to be computed accordingly in order to guarantee exploration. 
The value for $V_{max}$ is computed as $R_{max}/(1-\gamma)$ in the MAB domains, whereas $V_{max} = R_{max}$ 
in the Rotating Maze domain. 
Particularly in the MAB domains, the optimistic value is a discounted sum of rewards considering that, 
in the best case, the agent can be rewarded at every timestep. 
Therefore, an upper bound is set by multiplying the maximum reward $R_{max}$ by the expected number of future 
steps considered while computing the value function given the discount factor $1/(1-\gamma)$. 
In the Rotating Maze, however, an agent is only rewarded once it reaches the goal. 
Thus, a stricter upper bound on the value function is the actual undiscounted maximum reward $R_{max}$. 


\begin{table}[]
    \centering
    \small
    \begin{tabular}{@{}|r|r|r|r|@{}}
    \hline
    $m_0$ & $\delta$ & $\epsilon$ & \textit{Training episodes} \\ \hline
    1000 & 0.2   & 0.1     & 5000000           \\ \hline \addlinespace[0.1cm]
    \end{tabular}
    \caption{Parameters fixed throughout all experiments.}
    \label{tab:global-parameters}
\end{table}

Finally, Table~\ref{tab:global-parameters} shows parameters that are fixed throughout the experiments, 
independently of the domain. 
The first is the \texttt{RMax} parameter $m_0$, which defines the minimum count for a 
state-action pair to be considered as known by the \texttt{RMax} agent. 
There are definitions in the literature for computing $m_0$ in order to have guarantees 
\cite{strehl2009reinforcement}, but the resulting value is typically large. 
In our case, we set it to a constant $m_0=1000$ due to the fact that lower values leads \texttt{RMax} 
to exploit the safe parts of the abstraction earlier as they get available to the agent. 
The second and third parameters are confidence $\delta$ and accuracy $\epsilon$, respectively. 
Note that the confidence $\delta$ is halved during the execution of the \texttt{MarkovAbstraction}, 
such that half of it accounts for the confidence in the \texttt{RMax} agent, 
and the other half for the \texttt{StreamCPDFALearner} algorithm, as shown in Lines 1-2 of 
Algorithm \ref{alg:abstraction-module-complete}. 
The last parameter is the number of training episodes used in each run, which is set 
to $5$ million in order to make sure that we collect enough data to show convergence in each domain. 
Parameters not discussed in this section are set as defined in Table \ref{tab:quantities} of 
Appendix \ref{sec:algorithm-pseudocodes}.

\paragraph{Reproducibility and experimental setup.} 
The results shown in this paper are reproducible, and the definitions of our experiments are provided 
in the source code, along with the exact random seeds to reproduce the results. 
The source code contains instructions on how to run the reported experiments, 
as well as running experiments in general using our instantiation of Markov Abstractions. 
A virtual environment is available for running the code with its requirements. 
Our experiments were carried out in a server running Ubuntu 18.04.5 LTS, with 512GB RAM, 
and 80 cores model Intel Xeon E5-2698 2.20GHz. 
Each training run takes one core and the necessary amount of compute and time depends mostly on the number 
of episodes set for training. 


==> sections/problem.tex <==

\section{Reinforcement Learning}

We consider Reinforcement Learning (RL) as the problem of an agent that
has to learn an optimal policy for an unknown decision process $\rdp$, by acting
and receiving observation states and rewards according to the transition and
reward functions of $\rdp$.
The agent performs a sequence of actions $a_1 \dots a_L$,
receiving an observation $s_i$ and a reward $r_i$ after each action $a_i$.
The agent has a finite lifespan $L$. In particular, we will consider the case
when $L$ is a fixed constant (a.k.a.\ fixed horizon), and the case when the
agent has a constant probability of failure at each moment.\footnote{The
former case will be reduced to the markovian fixed-horizon setting, and the
latter case to the markovian discounted setting. Considering that a geomtric
distribution amounts to a discount \cite{puterman1994markov}.}
Thus, the interaction of the agent with the environment generates strings 
$a_1s_1r_1 \dots a_L s_L r_L$, called \emph{episodes}. They form the
\emph{experience} of the agent, upon which to learn.
Our focus is on learning a near-optimal policy. The agent is not required to
eventually follow such a policy, but simply to return it. 


